On the Interaction Between Differential Privacy and Gradient Compression in Deep Learning

While differential privacy and gradient compression are separately well-researched topics in machine learning, the study of interaction between these two topics is still relatively new. We perform a detailed empirical study on how the Gaussian mechanism for differential privacy and gradient compression jointly impact test accuracy in deep learning. The existing literature in gradient compression mostly evaluates compression in the absence of differential privacy guarantees, and demonstrate that sufficiently high compression rates reduce accuracy. Similarly, existing literature in differential privacy evaluates privacy mechanisms in the absence of compression, and demonstrates that sufficiently strong privacy guarantees reduce accuracy. In this work, we observe while gradient compression generally has a negative impact on test accuracy in non-private training, it can sometimes improve test accuracy in differentially private training. Specifically, we observe that when employing aggressive sparsification or rank reduction to the gradients, test accuracy is less affected by the Gaussian noise added for differential privacy. These observations are explained through an analysis how differential privacy and compression effects the bias and variance in estimating the average gradient. We follow this study with a recommendation on how to improve test accuracy under the context of differentially private deep learning and gradient compression. We evaluate this proposal and find that it can reduce the negative impact of noise added by differential privacy mechanisms on test accuracy by up to 24.6%, and reduce the negative impact of gradient sparsification on test accuracy by up to 15.1%.

==> content/tab/quick.tex <==
\begin{tabular}{rl}
  \toprule
  symbol & definition \\
  \midrule
     $x$ & variable   \\
  \bottomrule
\end{tabular}

==> ut-thesis/makefile <==
all:
	make ins ;\
	make doc ;\
	make tests ;\
	make zip ;\
	make tds

ins:
	cd ut-thesis ;\
	rm ut-thesis.cls ;\
	pdflatex ut-thesis.ins

doc:
	cd ut-thesis ;\
	pdflatex ut-thesis.dtx

tests:
	for example in test/* ; do \
		cp ut-thesis/ut-thesis.cls $$example ;\
		cd $$example ;\
		pdflatex main && pdflatex main && bibtex main && pdflatex main ;\
		rm ut-thesis.cls ;\
		cd ../../ ;\
	done

debug:
	cp ut-thesis/ut-thesis.cls test/.debug/ ;\
	cd test/.debug ;\
	pdflatex main && pdflatex main && bibtex main && pdflatex main ;\
	rm ut-thesis.cls ;\

zip:
	zip ctan/ut-thesis.zip \
		ut-thesis/ut-thesis.dtx \
		ut-thesis/ut-thesis.ins \
		ut-thesis/ut-thesis.pdf \
		ut-thesis/README

tds:
	mkdir -p .texmf/tex/latex/ut-thesis ;\
	mkdir -p .texmf/doc/latex/ut-thesis ;\
	cd .texmf ;\
	cp ../ut-thesis/ut-thesis.cls tex/latex/ut-thesis/ ;\
	cp ../ut-thesis/ut-thesis.pdf doc/latex/ut-thesis/ ;\
	cp ../ut-thesis/README doc/latex/ut-thesis/ ;\
	zip ut-thesis.tds.zip -r * ;\
	cp ut-thesis.tds.zip ../ctan ;\
	cd .. ;\
	rm -r .texmf

